FLECS-CGD: A Federated Learning Second-Order Framework via Compression and Sketching with Compressed Gradient Differences

In the recent paper FLECS (Agafonov et al, FLECS: A Federated Learning Second-Order Framework via Compression and Sketching), the second-order framework FLECS was proposed for the Federated Learning problem. This method utilize compression of sketched Hessians to make communication costs low. However, the main bottleneck of FLECS is gradient communication without compression. In this paper, we propose the modification of FLECS with compressed gradient differences, which we call FLECS-CGD (FLECS with Compressed Gradient Differences) and make it applicable for stochastic optimization. Convergence guarantees are provided in strongly convex and nonconvex cases. Experiments show the practical benefit of proposed approach.

==> graveyard.tex <==
&= \EE{Q}{F(w_{k})} - F^* - \alpha \lp \mu_1 - \ls \frac{L \alpha \mu_2^2 }{2}  \rs - c L \alpha \rp \EE{Q}{\|\nabla F(w_k)\|_2^2} +c \frac{L \alpha^2 \ls 1-\gamma_k \rs}{2n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2\\& + c \frac{L \alpha^2}{2} \gamma_k \zeta^2 + \underbrace{\ls \frac{L \alpha^2 \mu_2^2 }{2} \frac{\omega}{n} + c\frac{L \alpha^2(\gamma_k^2 \omega - \gamma_k (1-\gamma_k))}{2} \rs }_{\leq 0 \text{ by choice of $c$ and $\gamma_k$} } \frac{1}{n} \|\nabla f_i(w_k) - h_i^k \|_2^2

\begin{comment}

\begin{proof}
    We have $w_{k+1} = w_k - \alpha_k A_k \wg_k$, therefore:
    \begin{align*}
        \EE{Q}{F(w_{k+1})} &= \EE{Q}{F(w_k - \alpha_k A_k \wg_k)}\\
        &\stackrel{\eqref{assum:L-smoothness}}{\leq} \EE{Q}{F(w_{k})} - \alpha \EE{Q}{\la \nabla F(w_k), A_k \wg_k \ra} + \frac{L \alpha^2 }{2} \EE{Q}{\|A_k \wg_k\|^2}\\
        &\stackrel{\eqref{eq:bnd_Hess1},\eqref{eq:cg_lm1_1}}{\leq} \EE{Q}{F(w_{k})} - \alpha \mu_1 \EE{Q}{\|\nabla F(w_k)  \|^2} +   \frac{L \alpha^2 \mu_2^2 }{2} \EE{Q}{\|\wg_k\|^2}\\
        &= \EE{Q}{F(w_{k})} - \alpha \mu_1 \EE{Q}{\|\nabla F(w_k)  \|^2} +   \frac{L \alpha^2 \mu_2^2 }{2} \lp \EE{Q}{\|\wg_k - \nabla F(w_k) \|^2} + \EE{Q}{\|\nabla F(w_k)\|^2}\rp\\
        &\stackrel{\eqref{eq:cg_lm1_1}}{\leq} \EE{Q}{F(w_{k})} + \alpha\ls \frac{L \alpha \mu_2^2 }{2} -  \mu_1  \rs \EE{Q}{\|\nabla F(w_k)\|^2} + \frac{L \alpha^2 \mu_2^2 }{2} \frac{\omega}{n^2}\sum\limits_{i=1}^n \|\nabla f_i(w_k) - h_k^i\|^2
    \end{align*}\\
Define $\bk^k = F(w_k) - F^* + c \frac{L \alpha^2}{2}  \frac{1}{n} \sum_{i=1}^{n} \|h_i^{k} - h_i^* \|^2_2$
\begin{align*}
    \frac{1}{n} \sum_{i=1}^{n} \EE{}{\| h_i^{k+1} - h_i^* \|^2_2 | w_k} &\stackrel{\eqref{eq:error-feedback12}}{\leq} \frac{1}{n}  \sum_{i=1}^{n} \bigg[  \ls 1 - \gamma_k \rs \| h_i^k - h_i^*\|^2_2 + \gamma_k \|\nabla f_i(w_k) - h_i^* \|^2_2\\&+ \ls \gamma_k^2 \omega - \gamma_k (1-\gamma_k)\rs \|\nabla f_i(w_k) - h_i^k \|_2^2 \bigg] \\
    &= \frac{1-\gamma_k}{n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2 + \frac{\gamma_k}{n} \sum_{i=1}^{n} \|\nabla f_i(w_k) - h_i^* \|^2_2\\&+ \frac{\gamma_k^2 \omega - \gamma_k (1-\gamma_k)}{n} \sum_{i=1}^{n}  \|\nabla f_i(w_k) - h_i^k \|_2^2 \\
    &\leq  \frac{1-\gamma_k}{n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2 + \frac{2\gamma_k}{n}  \sum_{i=1}^n\| \nabla f_i(w_k) \|^2_2 + + \frac{2\gamma_k}{n}  \sum_{i=1}^n\| h_i^* \|^2_2\\&+ \frac{\gamma_k^2 \omega - \gamma_k (1-\gamma_k)}{n} \sum_{i=1}^{n}  \|\nabla f_i(w_k) - h_i^k \|_2^2 \\
    &\stackrel{\ref{asymmetry}}{\leq}  \frac{1-\gamma_k}{n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2 + 2 \gamma_k \|\nabla F(w_k) \|_2^2 + 4 \gamma_k \zeta^2\\&+ \frac{\gamma_k^2 \omega - \gamma_k (1-\gamma_k)}{n} \sum_{i=1}^{n}  \|\nabla f_i(w_k) - h_i^k \|_2^2 \\
\end{align*}
Therefore:
\begin{align*}
    \EE{}{\bk^{k+1}} &= \EE{}{F(w_k+1)} - f^* + c \frac{L \alpha^2}{2} \frac{1}{n} \sum_{i=1}^{n} \EE{}{\|h_i^{k+1} - h_i^* \|^2_2}\\
    &\leq  \EE{Q}{F(w_{k})} + \alpha\ls \frac{L \alpha \mu_2^2 }{2} -  \mu_1  \rs \EE{Q}{\|\nabla F(w_k)\|^2} + \frac{L \alpha^2 \mu_2^2 }{2} \frac{\omega}{n^2}\sum\limits_{i=1}^n \|\nabla f_i(w_k) - h_k^i\|^2 - F^*
    \\&  + c \frac{L \alpha^2}{2} \bigg[ \frac{1-\gamma_k}{n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2 + 2 \gamma_k \|\nabla F(w_k) \|_2^2 + 4 \gamma_k \zeta^2\\&+ \frac{\gamma_k^2 \omega - \gamma_k (1-\gamma_k)}{n} \sum_{i=1}^{n}  \|\nabla f_i(w_k) - h_i^k \|_2^2 \bigg]\\
    &= \EE{Q}{F(w_{k})} - f^* - \alpha \lp \mu_1 - \ls \frac{L \alpha \mu_2^2 }{2}  \rs - c L \alpha \rp \EE{Q}{\|\nabla F(w_k)\|_2^2} +c \frac{L \alpha^2 \ls 1-\gamma_k \rs}{2n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2\\& + c \frac{L \alpha^2}{2} \gamma_k \zeta^2 + \underbrace{\ls \frac{L \alpha^2 \mu_2^2 }{2} \frac{\omega}{n} + c\frac{L \alpha^2(\gamma_k^2 \omega - \gamma_k (1-\gamma_k))}{2} \rs }_{\leq 0 \text{ by choice of $c$ and $\gamma_k$} } \frac{1}{n} \|\nabla f_i(w_k) - h_i^k \|_2^2
\end{align*}

Therefore, we have: 
\begin{align*}
    \EE{}{\bk^{k+1}} &\leq \EE{Q}{F(w_{k})} - f^* - \alpha \underbrace{\lp \mu_1 - \ls \frac{L \alpha \mu_2^2 }{2}  \rs - c L \alpha \rp}_{\geq 0 \text{ by our choice of } \alpha} \EE{Q}{\|\nabla F(w_k)\|_2^2} +c \frac{L \alpha^2 \ls 1-\gamma_k \rs}{2n} \sum_{i=1}^{n}  \| h_i^k - h_i^*\|^2_2\\& + c \frac{L \alpha^2}{2} \gamma_k \zeta^2\\
    &\leq \EE{Q}{\bk^k} - \alpha \lp \mu_1 - \ls \frac{L \alpha \mu_2^2 }{2}  \rs - c L \alpha \rp \EE{Q}{\|\nabla F(w_k)\|_2^2} + c \frac{L \alpha^2}{2} \gamma_k \zeta^2  
\end{align*}

Therefore:
\begin{align*}
    \EE{Q}{\|\nabla F(w_k)\|_2^2} \leq 2 \frac{\EE{Q}{\bk^k} - \EE{Q}{\bk^{k+1}}}{ \alpha \ls 2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha\rs} +  \frac{cL \alpha}{2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha} \gamma_k \zeta^2
\end{align*}


Summing from $0$ and $k-1$ and simplifying the telescopic terms yiels:

\begin{align*}
   \sum_{j=0}^{k-1} \EE{Q}{\|\nabla F(w_j)\|_2^2} \leq 2 \frac{\bk^0 - \EE{Q}{\bk^{k}}}{ \alpha \ls 2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha\rs} + k \frac{cL \alpha}{2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha} \gamma_k \zeta^2
\end{align*}
Finally:
\begin{align}
    \frac{1}{k}\sum_{j=0}^{k-1} \EE{Q}{\|\nabla F(w_j)\|_2^2} \leq 2 \frac{\bk^0 - \EE{Q}{\bk^{k}}}{k \alpha \ls 2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha\rs} +  \frac{cL \alpha}{2\mu_1 - \ls L \alpha \mu_2^2  \rs - 2c L \alpha} \gamma_k \zeta^2
\end{align}
We can drop $\EE{Q}{\bk^k}$ because it is positive.
\end{proof}
\end{comment}
